ReSpec: Towards Optimizing Speculative Decoding in Reinforcement Learning Systems

Adapting large language models (LLMs) via reinforcement learning (RL) is often bottlenecked by the generation stage, which can consume over 75\% of the training time. Speculative decoding (SD) accelerates autoregressive generation in serving systems, but its behavior under RL training remains largely unexplored. We identify three critical gaps that hinder the naive integration of SD into RL systems: diminishing speedups at large batch sizes, drafter staleness under continual actor updates, and drafter-induced policy degradation. To address these gaps, we present ReSpec, a system that adapts SD to RL through three complementary mechanisms: dynamically tuning SD configurations, evolving the drafter via knowledge distillation, and weighting updates by rollout rewards. On Qwen models (3B--14B), ReSpec achieves up to 4.5x speedup while preserving reward convergence and training stability, providing a practical solution for efficient RL-based LLM adaptation.

==> sections/relatedwork.tex <==
\section{Related Work}

\noindent\textbf{RL Post-Training Frameworks.} A variety of frameworks have been proposed to accelerate RL post-training for LLMs. Early efforts~\cite{nemo, openrlhf, puzzle, deepspeedchat} focused on orchestrating the complex multi-stage workflow of RL post-training. More recent systems adopt architectural or scheduling innovations: VeRL~\cite{verl} introduces a hybrid-controller design to improve resource utilization, while DistFlow~\cite{distflow} employs a multi-controller approach to enhance scalability. RLHFuse~\cite{rlhfuse} fuses the generation and inference stages to reduce end-to-end training time, and RealHF~\cite{realhf} leverages optimized parallelism strategies to boost system throughput. To address long-tail rollouts, frameworks such as AReal~\cite{areal}, RollPacker \cite{rollpacker}, and RhymeRL~\cite{rhymesrl} adopt asynchronous post-training with tailored system optimizations to increase efficiency.  While existing RL post-training frameworks primarily focus on workflow orchestration, controller design, and system-level parallelism, they largely treat the generation stage as a black box and do not exploit SD. In contrast, \SysName specifically targets the generation bottleneck by integrating SD into RL training.


\noindent\textbf{Speculative Decoding.}
Speculative decoding (SD) has emerged as a widely studied technique to accelerate LLM generation. \cite{SD1,SD2} first proposed using a lightweight draft model to propose tokens, which are then validated by a stronger target model. Subsequent works extended this idea in various directions: Medusa~\cite{medusa} attaches multiple proposal heads to increase parallelism, Cascade Speculative Drafting~\cite{cascade} chains multiple draft–target stages for additional speedups. EAGLE\cite{eagle} leverages top-layer features of the target model as additional context and performs autoregression at the feature level, simplifying the drafting process. EAGLE-2~\cite{eagle2} estimates the acceptance rate using the confidence of the draft model and dynamically constructs a draft tree, pruning it at the end of the drafting stage. EAGLE-3~\cite{eagle3} further parallelizes the approach and fully supports the draft tree technique from EAGLE2, achieving state-of-the-art speedups in inference. Prior work on online speculative decoding (Online SD) has focused on inference-serving scenarios, where draft models are updated online to track shifting request distributions~\cite{distillspec,OSD}. In contrast, RL training requires the drafter to adapt to the evolving actor policy itself, posing unique challenges not addressed by existing Online SD methods.

